Operation Frames and Clubs in Kidney Exchange

A kidney exchange is a centrally-administered barter market where patients swap their willing yet incompatible donors. Modern kidney exchanges use 2-cycles, 3-cycles, and chains initiated by non-directed donors (altruists who are willing to give a kidney to anyone) as the means for swapping. We propose significant generalizations to kidney exchange. We allow more than one donor to donate in exchange for their desired patient receiving a kidney. We also allow for the possibility of a donor willing to donate if any of a number of patients receive kidneys. Furthermore, we combine these notions and generalize them. The generalization is to exchange among organ clubs, where a club is willing to donate organs outside the club if and only if the club receives organs from outside the club according to given specifications. We prove that unlike in the standard model, the uncapped clearing problem is NP-complete. We also present the notion of operation frames that can be used to sequence the operations across batches, and present integer programming formulations for the market clearing problems for these new types of organ exchanges. Experiments show that in the single-donation setting, operation frames improve planning by 34%--51%. Allowing up to two donors to donate in exchange for one kidney donated to their designated patient yields a further increase in social welfare.

==> arxiv version/hardness.tex <==
\begin{theorem}\label{thm:hardness}
The decision problem associated with the uncapped generalized clearing problem is NP-complete.
\end{theorem}
\begin{proof}[Proof sketch.]
   \noindent\emph{Membership in NP}: Given a set of mutually disjoint exchange clubs $\mathcal{C}$ and set of $k$ trades, it is trival to check in polynomial time if they satisfy Inequality~\ref{eq:nd}.

   \noindent\emph{NP-hardness}: We reduce from \textsc{SET-PACKING (SP)}.  An instance of \textsc{SP} takes a set of items $\mathcal{U}$, a family $\mathcal{S}$ of subsets of $\mathcal{U}$, and an integer $k$ as input; the task is to find a disjoint subfamily $\mathcal{X} \subseteq \mathcal{S}$ such that $|\mathcal{X}| = k$.

Assume that we are given an instance of \textsc{SP}.  We will now build an instance of our problem.  Let $n = |\mathcal{U}|$ be the number of items and $m = |\mathcal{S}|$ be the number of subsets.  Index the items $\{u_1, \ldots, u_n\} \in \mathcal{U}$ and the subsets $\{S_1, \ldots, S_m\} \in \mathcal{S}$.
%
Construct a disjoint set of clubs $\mathcal{C}$ as follows.  For each $u_i \in \mathcal{U}$, construct a club $a_i$ with no patient, one donor, and $\gamma_{a_i} = 1$.  For each subset $S_j \in \mathcal{S}$, construct a club $c_j$ with one patient and no donor.  Furthermore, for each subset $S_j$, construct a club $b_j$ with one donor and $\ell = |S_j|$ patients, $\gamma_{b_j} = 0$, and $\alpha_{b_j} = 1/\ell$.  Intuitively, this club will donate its one kidney iff each of the $\ell$ patients receives a kidney.

We now specify the set of legal transplants.  Let $M = |\mathcal{U}| + 1$.  For each subset $S_j \in \mathcal{S}$, draw a directed edge with weight $M$ from the single donor in club $b_j$ to the single patient in club $c_j$.  Furthermore, for each item $u_i \in \mathcal{U}$ and subset $S_j \in \mathcal{S}$ such that $u_i \in S_j$, draw one directed edge with weight $1$ from the single donor in club $a_i$ to the patient corresponding to item $u_i$ in club $b_j$.  Figure~\ref{fig:hardness} shows the final construction.
\begin{figure}[ht!bp]
%\vspace{-.15in}
\begin{subfigure}[b]{.38\linewidth}
\begin{center}
{\small Universe set:}\\
$\{1,2,3,4,5,6,7\}$\\
\vspace{2mm}
\small
{Set packing instance:}\\
\begin{tabular}{cc}
  \toprule
  $S_1$ & $\{1,3,4\}$\\
  $S_2$ & $\{1,3,5,7\}$\\
  $S_3$ & $\{4,6\}$\\
  \bottomrule
\end{tabular}
\end{center}
\caption{}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.60\linewidth}
\centering
\includegraphics[width=.92\linewidth]{asy/np_hardness.pdf}
\caption{}
\end{subfigure}
%\vspace{-.11in}
\caption{(b) Constructed instance of our problem. Each nodes represents a club, with donors in the top part, and patients in the bottom part. Edges represent compatibilities.}
\vspace{-.1in}
\label{fig:hardness}
\end{figure}

We will now show that a solution exists for the instance of \textsc{SC} if and only if our problem has a legal matching with weight in $[kM, (k+1)M)$.

\noindent
($\Rightarrow$)  Suppose there exists some solution $\mathcal{S'} = \{S'_1, \ldots, S'_k\}$ to the \textsc{SP} problem; that is, there exists some disjoint subfamily of $\mathcal{S}$ of size $k$.  Then, for each subset $S'_j \in \mathcal{S'}$, for each element $u_i$ in $S'_j$, use the edge from club $a_i$ to club $b_j$.  By the disjointness of the subfamily $\mathcal{S'}$, each single-donor club $a_i$ for $i \in [n]$ donates to at most one club.  Furthermore, each club $b_j$ corresponding to $S'_j \in \mathcal{S}'$ receives one kidney for each patient in its club; by construction, their matching multiplier is now satisfied.  Thus, for each $S'_j \in \mathcal{S'}$, include the edge with weight $M$ from the one donor in $b_j$ to the one patient in $c_j$.  This results in a matching of weight at least $kM$, but no more than $kM + n < (k+1)M$.

\noindent
($\Leftarrow$)  Suppose there exists a matching in our problem such that the weight of the matching is in $[kM, (k+1)M)$.  Then exactly $k$ of the edges between exactly $k$ pairs of clubs $b_\cdot$ and $c_\cdot$ are used, at total weight $kM$.  Let $j' \in [m']$ index those clubs $b_{j'}$ that use their one outgoing edge to club $c_{j'}$.  Each club $b_{j'}$ uses that edge if and only if every one of its internal patients receives a kidney; since each single-donor club $a_\cdot$ can give at most one kidney, they are used at most once.  Since at most $n$ clubs $a_\cdot$ can be used, each at additional weight $1$, the final matching is of weight at most $km+n < (k+1)M$; further, exactly $k$ clubs $b_{j'}$ were fulfilled completely, corresponding to exactly $k$ disjoint subsets $S_{j'} \in \mathcal{S}$ being packed.
\end{proof}

